Limits on the Stochastic Gravitational Wave Background from the North American Nanohertz Observatory for Gravitational Waves

We present an analysis of high-precision pulsar timing data taken as part of the North American Nanohertz Observatory for Gravitational waves (NANOGrav) project. We have observed 17 pulsars for a span of roughly five years using the Green Bank and Arecibo radio telescopes. We analyze these data using standard pulsar timing models, with the addition of time-variable dispersion measure and frequency-variable pulse shape terms. Sub-microsecond timing residuals are obtained in nearly all cases, and the best root-mean-square timing residuals in this set are ~30-50 ns. We present methods for analyzing post-fit timing residuals for the presence of a gravitational wave signal with a specified spectral shape. These optimally take into account the timing fluctuation power removed by the model fit, and can be applied to either data from a single pulsar, or to a set of pulsars to detect a correlated signal. We apply these methods to our dataset to set an upper limit on the strength of the nHz-frequency stochastic supermassive black hole gravitational wave background of h_c (1 yr^-1) < 7x10^-15 (95%). This result is dominated by the timing of the two best pulsars in the set, PSRs J1713+0747 and J1909-3744.

==> rms_table.tex <==
\begin{tabular}{c|rr|r|r}
\hline
Source & Multi-channel & $\chi^2$ & Epoch averaged & High-freq averaged\\
 & RMS, $\mu$s & & RMS, $\mu$s & RMS, $\mu$s \\
\hline
J1713+0747 & 0.106 & 1.48 & 0.030 & 0.041 \\
J1909--3744 & 0.181 & 1.95 & 0.038 & 0.047 \\
B1855+09   & 0.395 & 2.19 & 0.111 & 0.101 \\
J0030+0451 & 0.604 & 1.44 & 0.148 & 0.328 \\
J1600--3053 & 1.293 & 1.45 & 0.163 & 0.141 \\
J0613--0200 & 0.781 & 1.21 & 0.178 & 0.519 \\
J1744--1134 & 0.617 & 3.58 & 0.198 & 0.229 \\
J2145--0750 & 1.252 & 1.97 & 0.202 & 0.494 \\
J1918--0642 & 1.271 & 1.21 & 0.203 & 0.211 \\
J2317+1439 & 0.496 & 3.03 & 0.251 & 0.155 \\
J1853+1308 & 1.028 & 1.06 & 0.254 & 0.271 \\
J1012+5307 & 1.327 & 1.40 & 0.276 & 0.345 \\
J1640+2224 & 0.562 & 4.36 & 0.409 & 0.601 \\
J1910+1256 & 1.394 & 2.09 & 0.708 & 0.710 \\
J1455--3330 & 4.010 & 1.01 & 0.787 & 1.080 \\
B1953+29   & 3.981 & 0.98 & 1.437 & 1.879 \\
J1643--1224 & 2.892 & 2.78 & 1.467 & 1.887 \\
\hline
\end{tabular}

